Climate data selection for multi-decadal wind power forecasts

Reliable wind speed data is crucial for applications such as estimating local (future) wind power. Global Climate Models (GCMs) and Regional Climate Models (RCMs) provide forecasts over multi-decadal periods. However, their outputs vary substantially, and higher-resolution models come with increased computational demands. In this study, we analyze how the spatial resolution of different GCMs and RCMs affects the reliability of simulated wind speeds and wind power, using ERA5 data as a reference. We present a systematic procedure for model evaluation for wind resource assessment as a downstream task. Our results show that higher-resolution GCMs and RCMs do not necessarily preserve wind speeds more accurately. Instead, the choice of model, both for GCMs and RCMs, is more important than the resolution or GCM boundary conditions. The IPSL model preserves the wind speed distribution particularly well in Europe, producing the most accurate wind power forecasts relative to ERA5 data.

==> editor_letter.tex <==
%\documentclass{article}
%\usepackage{graphicx} % Required for inserting images

\date{July 2024}

%\begin{document}\noindent
Dear editors,

I am enclosing our paper, "Climate data selection for multi-decadal wind power forecasts." We investigate which climate data and spatial resolution most accurately represent wind speeds for multi-decadal wind power predictions.

We evaluate the reliability of projected wind speeds from various GCMs and RCMs, using ERA5 data as a reference.
Given the challenge of evaluating climate model data that is not spatio-temporally aligned, we propose a systematic evaluation procedure that quantifies differences in wind speed distributions and cumulative multi-decadal wind power predictions. Our findings reveal that GCMs and RCMs of higher spatial resolution do not necessarily preserve wind speeds more accurately. Instead, we find that the choice of model for GCMs and RCMs is more important than the spatial resolution. For RCMs, we also find that the model choice is more important than the GCM boundary conditions. Notably, the IPSL model preserves the wind speed distribution particularly well in Europe relative to ERA5 data, resulting in the most accurate wind power predictions.

Previous research published in ERL investigated the influence of the temporal resolution of wind speeds on multi-decadal predictions (Effenberger et al., 2024). It revealed that systematic errors can be introduced by insufficient temporal resolution or by averaging wind speeds. Building on these insights, we investigate the spatial resolution of climate models. We find that, in contrast to the temporal resolution, there is no spatial climate model resolution that overcomes systematic errors in wind speeds. Additionally, we present an approach to evaluate wind data for multi-decadal predictions which is applicable to other data and could, for example, be used to analyze bias-corrected data. Our research provides valuable insights to the climate science community as our work emphasizes the importance of climate model choice over spatial resolution. 

The keywords for our submission are: spatial resolution, climate models, wind speed, wind power.


All the data used in this study are open-source. Upon acceptance of our manuscript, we will make the code available on GitHub. As the corresponding author, I confirm that all co-authors have approved the submission of this manuscript to Environmental Research Letters and that it has not been submitted or published elsewhere.

If you require any additional information, please do not hesitate to contact me.

Sincerely,

Sofia Morelli

sofia.morelli@uni-tuebingen.de
\newpage

%\end{document}

